Improved Algorithms for Fully Dynamic Maximal Independent Set

Maintaining maximal independent set in dynamic graph is a fundamental open problem in graph theory and the first sublinear time deterministic algorithm was came up by Assadi, Onak, Schieber and Solomon(STOC'18), which achieves $O(m^{3/4})$ amortized update time. We have two main contributions in this paper. We present a new simple deterministic algorithm with $O(m^{2/3}\sqrt{\log m})$ amortized update time, which improves the previous best result. And we also present the first randomized algorithm with expected $O(\sqrt{m}\log^{1.5}m)$ amortized time against an oblivious adversary.

==> arboricity.tex <==

\section{An $O(\sqrt{m\log m}\lambda^{\frac{3}{2}})$-Update-Time algorithm}

\begin{defn}
A graph G=(V,E) has arboricity $\lambda$ if $$\lambda=\max_{U\subseteq V} \left\lceil\frac{|E(U)|}{|U|-1}\right\rceil,$$ where $E(U)$ is the set of edges induced by $U$ (we only consider about $|U|\geq 2$).
\end{defn}

It is a useful property that if a graph $G$ has arboricity $\lambda$, then every sub-graph of $G$ has arboricity at most $\lambda$. And another key property which is extensively used in other algorithmic applications is given by Nash-Williams \cite{nash1961edge}, \cite{nash1964decomposition}.

\begin{theorem}
A graph $G$ has arboricity $\lambda$ if and only if $\lambda>0$ is the smallest number such that $G$ can partition edges into $\lambda$ sets and each set forms a forest.
\end{theorem}

This theorem has a direct corollary.

\begin{cor}\label{corxx}
If a graph $G=(V,E)$ has arboricity $\lambda$, then there is an orientation of edges such that the out-degree of each vertex is at most $\lambda$. An orientation is to assign a direction to every edge $e \in E$.
\end{cor}


For bounded arboricity graph, we show a deterministic algorithm which runs in $O(\sqrt{m\log m}\lambda^{\frac{3}{2}})$ time. In another word, for low arboricity graphs (e.g. planar graphs, bounded tree-width graphs, and all excluded-minor graphs), we get a $O(\sqrt{m\log m})$ result, which is near $O(\sqrt{m})$. As we explain in the section \ref{hardness}, $o(\sqrt{m})$ is somehow a barrier even in a fully dynamic forest if we are required to show MIS explicitly.

Like the above two algorithms, this algorithm also separate the whole edge update sequence into several epochs. In each epoch, the algorithm will call \textit{reconstruction part} to reconstruct the MIS and whole data structures and then call \textit{running part} to deal with the following edge updates. All following analysis is in one epoch. For clarity, we emphasize that all notations with $*$ means that it will remain unchanged during the \textit{running part} after being defined in \textit{reconstruction part}, like $V_{high}^*$.

\subsection{Preliminary}
\textbf{Notation.} Let $G=(V,E)$ be the graph, $m=|E|$ is the number of edges, $\mathcal{M}$ is the MIS we are maintaining. $\text{deg}(v)$ is the degree of vertex $v$. $N(v)$ is the set of $v$'s neighbor and we can define $N(S)=\cup_{v\in S}N(v)$ for simplicity.

Consider the beginning of an epoch. Let $T=\sqrt{m\log m\cdot\lambda}$ be the number of edge updates we should handle in the future, and let $V_{high}^*=\{v\in V|\text{deg}(v)\geq 20T\}$. Denote $A=N(V_{high}^*)\setminus V_{high}^*$ which will change by time. And denote $A^*=N(V_{high}^*)\setminus V_{high}^*$ which is fixed. Like the algorithm in section \ref{section_alg_1}, our main technique to bound the running time is to have the following invariant at the end of each edge update.

\begin{inv}\label{inv1}
All vertices in $V_{high}^*$ has at least one neighbor in $\mathcal{M}$.
\end{inv}

We can keep this invariant by maintaining an \textbf{injection} $f:V_{high}^*\rightarrow A$ (i.e. $f(v_i)$ is different from each other) such that $\forall v,~f(v)\in \mathcal{M}$. The maintenance of $\mathcal{M}$ will become trivial if this invariant holds since only those low-degree vertices will change their state of whether it is in $\mathcal{M}$. But the problem occurs when this invariant is broken. For example, the adversary add an edge between $f(v_1)$ and $f(v_2)$. In this case, we must remove one of them from $\mathcal{M}$, say $f(v_1)$ is removed. To keep the invariant, we must force one of $v_1$'s neighbor, say $u$, join $\mathcal{M}$, along with the cost that all vertices in $\mathcal{M}$ which is also the neighbor of $u$ should be removed from $\mathcal{M}$. After a bunch of vertices being removed, we should check their neighbors whether they should join $\mathcal{M}$ due to the maximality of $\mathcal{M}$. And this situation can occur in every edge updates. In the \textit{reconstruction part}, we will assign every vertex in $V_{high}^*$ a \textit{level} to help us analyze.

%{\color{red}{[$A$ or $A^*$?]}}

\subsection{Reconstruction part}


\begin{algorithm}
\caption{Stage 1}\label{stage1}
\begin{algorithmic}
\State $K_1\gets V_{high}^*$
\For{$i\gets 1$ to $\lceil \log m \rceil$}
\State $\text{unitcost}_i(u)\gets \frac{\text{deg}(u)}{|N(u)\cap K_i|}$, $\forall u\in A^*$.
\State $S_i(v)\gets  \{\text{unitcost}_i(u)\mid u\in N(v)\cap A^*\}$. ($S_i(v)$ is a multiset).
\State $p(v)\gets \text{median number among}$ $S_i(v)$, $\forall v\in K_i$.
\State $L_i\gets \{v\in K_i \mid p(v) \leq \frac{m}{|K_i|\cdot T}\}$.
\State $level^*(v)\gets i$, $\forall v\in L_i$.
\State $candidate^*(v)\gets \{u\in N(v)\cap A^*\mid\text{unitcost}_i(u)\leq p(v) \}$, $\forall v\in L_i$.
\State $K_{i+1}\gets K_i\setminus L_i$.
\EndFor
\end{algorithmic}
\end{algorithm}


Here we brief explain things we do in algorithm \ref{stage1}. To keep the invariant $\ref{inv1}$, it is necessary to choose $f(.)$ for every vertices in $V_{high}^*$. But we cannot decide $f(v)$ to be an arbitrary neighbor, since $\{f(v)\}$ is also an independent set in the graph. To see a bad case, one may decide $f(v)$ in some order, denote it $\{v_1,...,v_{|V_{high}^*|}\}$. When processing on $v_i$, maybe all of $v_i$'s neighbor has one neighbor in $\{f(v_1),...,f(v_{i-1})\}$, then the process stuck. Notice that $deg(u)$ is a good measurement for $v\in V_{high}^*$ to choose their $f(v)$. The less $deg(f(v))$ is, the less possibility the process stuck.

In each level $i$, we divide the value of $deg(u)$ into $|N(u)\cap K_i|$ part which called unitcost$_i(u)$ and allocate each part to the list $S_i(v)$ for all $v\in N(u)\cap K_i$. For each $v\in K_i$, neighbors with small unitcost$_i$ are good candidates for $v$ to choose $f(v)$. If $v$ has many such candidates, we put $v$ into level $i$ and do the same process for the remained.

\begin{lemma}
After the algorithm \ref{stage1} finish the for-loop, all vertices in $V_{high}^*$ will have their own $level^*(.)$. In another word, $K_{\lceil \log m\rceil+1}=\emptyset$.
\end{lemma}

\proof In iteration $i$, the following inequality holds. $$4T\sum_{v\in K_i}p(v)\leq \sum_{v\in K_i}\sum_{val\in S_i(v)}val\leq \sum_{u\in A^*}deg(u)\leq 2m.$$ The first inequality is correct because that $p(v)$ is the median number of $S_i(v)$ and $|S_i(v)|\geq \text{deg}(v)-|V_{high}^*|\geq 8T$. The second inequality follows that every $u\in A^*$ separate its deg$(u)$ into $|N(u)\cap K_i|$ parts which is the definition of unitcost$(u)$, and allocate each part to $S_i(v)$ where $v\in N(u)\cap K_i$.

So the average value among $p(v)$ is at most $\frac{m}{2|K_i|T}$, thus $L_i$ will occupy at least half of $K_i$, $K_{i+1}$ will shrink by a factor of 2. $\hfill\square$

In the remainder of this \textit{reconstruction part}, we should choose $f(.)$ for every vertices in $V_{high}^*$ in order to keep the invariant, then we can finish the \textit{reconstruction part} by checking other vertices one by one to ensure the maximality of $\mathcal{M}$ and start the \textit{running part}.

\begin{lemma}\label{mainlemma}
After the graph takes t ($t\leq T$) edge updates, $\forall f:V_{high}^*\rightarrow V$ s.t. $f(v)\in candidate^*(v)$ and $f(v)$ is different from each other, $\sum_{v\in V_{high}^*}\text{deg}(f(v))\leq 4T$.
\end{lemma}
\proof We first consider the case that $t=0$, and then consider the vertices in $V_{high}^*$ level by level. For level $i$, $\forall v\in L_i$, unitcost$_i(f(v))\leq \frac{m}{|K_i|\cdot T}$ since $f(v)\in candidate^*(v)$ and by definition of $L_i$. Thus $$\sum_{v\in L_i}deg(f(v))=\sum_{v\in L_i}\text{unitcost}_i(f(v))\cdot |N(f(v))\cap K_i|\leq \frac{m}{|K_i|\cdot T}\sum_{v\in L_i}|N(f(v))\cap K_i|.$$ The right most term $\sum_{v\in L_i}|N(f(v))\cap K_i|$ is exactly the number of edges between $f(L_i)$ and $K_i$ in their induced graph, which is at most $2\lambda|K_i|$. So $$\sum_{v\in V_{high}^*}\text{deg}(f(v))\leq 2\sqrt{m\log m\cdot \lambda}=2T.$$ After the graph takes $t$ edge updates, $\sum_{v\in V_{high}^*}\text{deg}(f(v))$ will at most increase by $2t$ compare to the case that $t=0$. Thus it is at most $4T$.

$\hfill\square$

Using Lemma \ref{mainlemma}, we can decide from $f(v_1)$ to $f(v_{|V_{high}^*|})$ one by one. When processing on $v_i$, we can choose one neighbor in $candidate^*(v_i)$ that has no neighbor in $\{f(v_1),...,f(v_{i-1})\}$ as our $f(v_i)$. Such neighbor always exist since $v_i$ has more than $20T$ neighbors and $\sum_{j<i}deg(f(v_j))\leq 4T$ by lemma \ref{mainlemma}.

There are $O(\log m)$ steps in the $for-loop$, and each loop can be done in linear time. So the total reconstruct time complexity is $O(m\log m)$. After allocating into $T$ edge updates, we get an $O(\frac{m\log m}{T})<O(\lambda T)$ amortized time reconstruction.

\subsection{Running part}
We maintain the following information:

\noindent\begin{minipage}[c]{1.0\textwidth}
\fbox{
\parbox{\textwidth}{
\begin{itemize}
\setlength{\itemsep}{0pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
\item[$\bullet$] For every $v\in V$, \texttt{MIS-counter[v]}$=|N(v)\cap \mathcal{M}|$, which means the number of $v$'s neighbors in the MIS.
\item[$\bullet$] For every $v\in A^*$, \texttt{replace-cost[v]}$=\sum_{u\in N(v)\cap \mathcal{M}}\text{deg}(u)$, which means the total degree of $v$'s neighbors in the MIS. We only maintain this information for vertices in $A^*$. Recall that $A^*=N(V_{high}^*)\setminus V_{high}^*$. It is defined at the beginning of this epoch and remain unchanged during the edge updates.
\item[$\bullet$] For every $v\in V_{high}^*$, \texttt{feasible[v]} is a list containing all vertices in $candidate^*(v)\cap N(v)$ which has no neighbor in $\{f(v)\mid v\in V_{high}^*\}$.
\end{itemize}
}
}
\end{minipage}

We assume that we will update the above information as soon as an edge is inserted/deleted or some vertex changes its state of whether it is in $\mathcal{M}$.

Instead of maintaining invariant \ref{inv1}, our algorithm will keep a stronger invariant at the end of each edge update, which can directly imply invariant \ref{inv1}.

\begin{inv}\label{inv2}
For every $v\in V_{high}^*$, there is $f(v)\in N(v)\cap candidate^*(v)$ such that $f(v)\in \mathcal{M}$. And $f(v_i)$ is different from each other.
\end{inv}

Obviously, this invariant \ref{inv2} is held at the time that we finish the \textit{reconstruction part} and no edge update occurs.

We now have the following straightforward property.

\begin{claim}\label{claim1}
If invariant \ref{inv2} holds, then the size of \texttt{feasible[v]} is always larger than $5T$ for all $v\in V_{high}^*$.
\end{claim}
\proof Consider a vertex $u$ in $candidate^*(v)$, there are two reasons that $u$ cannot be in \texttt{feasible[v]}. One is that it is no long a neighbor of $v$ due to an edge deletion, or $u$ has a neighbor in $f(V_{high}^*)$. There are at most $T$ vertices for the first reason and at most $4T$ vertices for the second which is the statement of lemma \ref{mainlemma}. Thus $|\texttt{feasible[v]}|\geq 10T-T-4T\geq 5T$.$\hfill\square$

Let's only consider how vertices change their state of whether it is in $\mathcal{M}$ or not when an edge got updated, and leave the time complexity of maintaining \texttt{MIS-counter[v]}, \texttt{replace-cost[v]} and \texttt{feasible[v]} in the Analysis section.

\subsubsection{Edge Deletions}

Assume now an edge $e=(u,v)$ get removed.

\noindent\textbf{Case 1:} Neither $u$ or $v$ is in $\mathcal{M}$. In this case, nothing happens.

\noindent\textbf{Case 2:} One of $u$ and $v$ is in $\mathcal{M}$. We assume it is $u$ w.l.o.g. We simply check whether \hbox{\texttt{MIS-counter[v]}} becomes $0$ after removing this edge. If so, let $v$ join $\mathcal{M}$.

\subsubsection{Edge Insertions}

Assume now an edge $e=(u,v)$ is inserted.

\noindent\textbf{Case 1:} At most one of $u,v$ is in $\mathcal{M}$. In this case, nothing happens.

\noindent\textbf{Case 2:} Both $u$ and $v$ are in $\mathcal{M}$. Thus we must remove one of them from $\mathcal{M}$. We continue to divide this case into two sub-cases.

\textbf{Case 2-a:} One of $u,v$ is not in $f(V_{high}^*)$. Assume this vertex is $u$. Removing $u$ from $\mathcal{M}$ won't break the invariant \ref{inv2}. So we can just do it and enumerate $u$'s neighbor one by one to check if their \texttt{MIS-counter[.]}$=0$. If so, we add it to $\mathcal{M}$ and continue the enumeration. One can easily verify that the maximality of $\mathcal{M}$ is still preserved after the enumeration.

\textbf{Case 2-b:} Both $u$ and $v$ are in $f(V_{high}^*)$. Thus we must remove one of them from $\mathcal{M}$ and the invariant \ref{inv2} is no longer held. Assume the vertex we removed is $u$, and the corresponding vertex in $V_{high}^*$ respect to $f(.)$ is $x$. We must find a replacement of $f(x)$ in order to keep the invariant \ref{inv2}.

\begin{lemma}\label{replacelemma}
For any $S\subseteq A^*$ s.t. $|S|\geq 5T$, there exists $y\in S$ such that \texttt{replace-cost[y]}$\leq 22\lambda T$.
\end{lemma}

\proof From Corollary \ref{corxx} we know there exists an edge orientation of $E$ s.t. the out-degree of each vertex is at most $\lambda$. For all $y\in S$, we divide \texttt{replace-cost[y]}$=\sum_{u\in N(v)\cap \mathcal{M}}\text{deg}(u)$ into two parts according to this edge orientation, denoted by in-part and out-part. For out-part, we only consider the neighbors of $y$ connected with an out-edge and it will contribute at most $21\lambda T$ since there are at most $\lambda$ out-edges and every vertex in $\mathcal{M}$ has degree at most $21T$. For every vertex in $\mathcal{M}$, it has at most $\lambda$ out-edges and their total degree is $2m$. Since $|S|\geq 5T$, the minimum in-part among $S$ is at most $\frac{2\lambda m}{5T}\leq T$. Combine these two part, we know there exists $y\in S$ such that \texttt{replace-cost[y]}$\leq 22\lambda T$. $\hfill\square$

Combine the result of claim \ref{claim1} and lemma \ref{replacelemma}, we can find such $y$ by enumerate at most $5T$ vertices in \texttt{feasible[x]}. Then we can force $y$ to join $\mathcal{M}$ and remove all its neighbor along with $u$ from $\mathcal{M}$, and let $f(x)\gets y$. Then do the check for all neighbors of those vertices removed from $\mathcal{M}$ to ensure the maximality, like the things we do in case 2-a.

\subsubsection{Analysis About Running Time}

Recall that we should maintain the information about \texttt{MIS-counter}, \texttt{replace-cost}, \texttt{feasible} directly after an edge is inserted/deleted or some vertex join/leave $\mathcal{M}$. When an edge update happens, we can maintain them in $O(1)$. When some vertex $v$ join or leave $\mathcal{M}$, we should update the information of its neighbors and it will cost $O(deg(v))$ time. On the other hand, we will enumerate all $v$'s neighbor to ensure the maximality of $\mathcal{M}$ when $v$ got removed from $\mathcal{M}$, which will cost $O(deg(v))$ time. So naturally we define $\Phi=-\sum_{v\in \mathcal{M}}deg(v)$ as our potential function and the total running time in the $T$ rounds is bounded by the variation of $\Phi$ in the $T$ rounds.

\begin{claim}\label{cc}
$\Phi$ will increase by at most $22\lambda T$ in each round.
\end{claim}

\proof The impact of the decrease of $deg(v)$ for some $v\in \mathcal{M}$ is negligible. The main term is due to that some vertices leave $\mathcal{M}$, which occurs in either Case 2-a or Case 2-b. In Case 2-a, only one vertex $v$ leave and $deg(v)$ is at most $21T$ since $v\notin V_{high}^*$. In case 2-b, there can be a bunch of vertices leaving $\mathcal{M}$ but the total degree is bounded by $22\lambda T$. This is because that we choose a vertex $y$ with \texttt{replace-cost[y]}$\leq 22\lambda T$ and the definition of \texttt{replace-cost[y]} is exactly the total degree we loose. $\hfill\square$

With the result of Claim \ref{cc}, and the fact that $\Phi$ has an lower bound of $-2(m+T)$, we know the variation of $\Phi$ is at most $O(\lambda T^2+m)$, with $O(\lambda T)$ per round. And since we use $O(\lambda T)$ amortized time in the \textit{reconstruction part}, plug in to $T=\sqrt{m\log m\cdot\lambda}$ we get the following theorem as our result.

\begin{theorem}
Starting from an empty graph on n fixed vertices, and provided that the graph has arboricity at most $\lambda$ at all time. A maximal independent set can be maintained deterministically over any sequence of edge insertions and deletions in $O(\sqrt{m\log m}\lambda^{\frac{3}{2}})$ amortized update time, where m denotes the number of edge updates.
\end{theorem}

